Using Grammar Patterns to Interpret Test Method Name Evolution

It is good practice to name test methods such that they are comprehensible to developers; they must be written in such a way that their purpose and functionality are clear to those who will maintain them. Unfortunately, there is little automated support for writing or maintaining the names of test methods. This can lead to inconsistent and low-quality test names and increase the maintenance cost of supporting these methods. Due to this risk, it is essential to help developers in maintaining their test method names over time. In this paper, we use grammar patterns, and how they relate to test method behavior, to understand test naming practices. This data will be used to support an automated tool for maintaining test names.

==> archive.tex <==
\vspace{0.5mm}\subsubsection{What grammar patterns are typically found as prefixes to test method names?}

\begin{table*}[!ht]
%\fontsize{7.5}{10}\selectfont
\centering
\caption{Top 5 frequently occurring starting prefix grammar patterns for terms in a method's name before and after a rename.}
\label{Table:RenameGrammarPatternOldNew}
\begin{tabular}{lrrlrr}
\hline
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Old Grammar Pattern\end{tabular}}} & \multicolumn{1}{c}{\textbf{Count}} & \multicolumn{1}{c}{\textbf{Percentage}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}New Grammar Pattern\end{tabular}}} & \multicolumn{1}{c}{\textbf{Count}} & \multicolumn{1}{c}{\textbf{Percentage}} \\ \hline
\multicolumn{6}{c}{\textit{\begin{tabular}[c]{@{}c@{}}\\ Top 5 starting 2-prefix part of speech tag patterns for old and new names\end{tabular}}} \\
V V & 229 & \multicolumn{1}{r|}{39.01\%} & V NM & 173 & 29.03\% \\
V NM & 146 & \multicolumn{1}{r|}{24.87\%} & V V & 167 & 28.02\% \\
V N & 72 & \multicolumn{1}{r|}{12.27\%} & V N & 77 & 12.92\% \\
NM N & 38 & \multicolumn{1}{r|}{6.47\%} & NM N & 50 & 8.39\% \\
N V & 16 & \multicolumn{1}{r|}{2.73\%} & V P & 21 & 3.52\% \\
\textit{Others} & 86 & \multicolumn{1}{r|}{14.65\%} & \textit{Others} & 108 & 18.12\% \\
\multicolumn{6}{c}{\textit{\begin{tabular}[c]{@{}c@{}}\\ Top 5 starting 3-prefix part of speech tag patterns for old and new names\end{tabular}}} \\
V NM N & 135 & \multicolumn{1}{r|}{27.61\%} & V NM N & 159 & 31.99\% \\
V V NM & 95 & \multicolumn{1}{r|}{19.43\%} & V V NM & 77 & 15.49\% \\
V V N & 40 & \multicolumn{1}{r|}{8.18\%} & V V N & 30 & 6.04\% \\
V V P & 28 & \multicolumn{1}{r|}{5.73\%} & V V P & 20 & 4.02\% \\
V N P & 16 & \multicolumn{1}{r|}{3.27\%} & V N V & 17 & 3.42\% \\
\textit{Others} & 175 & 35.79\% & \textit{Others} & 194 & 39.03\% \\
\multicolumn{6}{c}{\textit{\begin{tabular}[c]{@{}c@{}}\\ Top 5 starting 4-prefix part of speech tag patterns for old and new names\end{tabular}}} \\
V NM NM N & 42 & \multicolumn{1}{r|}{17\%} & V NM NM N & 44 & 18\% \\
V V NM   NM & 33 & \multicolumn{1}{r|}{13\%} & V V NM   NM & 21 & 9\% \\
V V NM N & 22 & \multicolumn{1}{r|}{9\%} & V NM NM NM & 14 & 6\% \\
V NM NM   NM & 12 & \multicolumn{1}{r|}{5\%} & V V NM   N & 14 & 6\% \\
V V NM NPL & 11 & \multicolumn{1}{r|}{4\%} & V NM N VM & 7 & 3\% \\
\textit{Others} & 127 & \multicolumn{1}{r|}{51\%} & \textit{Others} & 139 & 58\% \\ \hline
\end{tabular}
\end{table*}

When examining the first part of speech tag for method names, we observe that a majority of both old and new names utilize a verb as the first term in the name. For example in the test method named \texttt{testComplexTable} \cite{rq01-x-01}, the starting term, `test' is a verb. In total, 527 (or approximately 85.69\%) old names, while 517 (or approximately 84.07\%) new names started with a verb. This phenomenon confirms coding standards recommendations of utilizing a strong verb followed by an object \cite{McConnell2004Book}. It also confirms findings in a prior study that examined the part of speech tags in production code \cite{Newman2020JSS}. Additionally, since our study is based on unit test methods, the term `test' is the most frequent verb utilized by developers as the starting term for the method's name. We also observe instances where the method name starts with a preposition; 8 (or approximately 1.30\%) old names and 6 (or approximately 0.98\%) new names. A manual examination of these methods shows that these methods are utilized as test fixtures. by developers (e.g., \texttt{before} \cite{rq01-x-02}).

In Table \ref{Table:RenameGrammarPatternOldNew}, we provide the top 5 starting part of speech prefix patterns for old and new names. Looking at at this table, we can see developers utilize a variety of parts of speech patterns when naming test methods. These patterns include verb phrases (i.e., \textit{V NM N}), noun phrases (i.e., \textit{NM N}), and dual verb phrases (i.e., \textit{V V NM}).

Similar to a study on production methods \cite{Newman2020JSS}, we observe that developers frequently utilize verb phrases when naming test methods. In this pattern, a verb is followed by a noun phrase. From this pattern, the noun phrase can inform us of the scenario under test. Using the prior example, \texttt{testComplexTable}, we observe that the method name starts with a verb (`text'), followed by an adjective or noun modifier (`Complex') and a noun (`Table').

The \textit{NM N}, or noun phrase pattern is either used by its self or as part of a verb phrase. This pattern consists of an adjective or noun modifier (\textit{NM}) followed by a noun (\textit{N}). In this pattern, the noun, also known as the head-noun, indicates the object or scenario under test. The adjective or noun modifier specifies characteristics or context around the test. An example of this pattern is the test method name \texttt{nullName} \cite{rq02_a_02}.

Looking at instances that start with two or more verbs (\textit{V V}), we see that, in most cases, the fist verb corresponds to the term `test' while the following verbs are part of the production method that the developer is testing. For example, in commit \cite{rq02_a_03}, the name of the test method is \texttt{testGetRemetente}. When we look at the code, we see that the test method is testing the output of a production method called \texttt{getRemetente}.

==> temp.tex <==

1) Since the purpose of test methods are to test atomic units of the code, the test method names are very specific to their intended behavior --- hence the naming structure differs from prod (e.g., 1030323,927666) -- developers try to describe the test using natural language
2) There are terms that are domain/technology/SE specific (testAndAggregation -- AND might not be a conjunction 546152)
 3) In certain instances, the surrounding code (and comments) would need to be reviewed to determine the pos tag -- 975156,285496
4) setup and teardown should be one term, but developers use camel casing which would cause splitters to inaccurately split the name (preamble)
5) nonsensical or not good test names -- 298503
6) expand contractions don't-->do not ---155066
7) sometimes the noun appears before the noun modifier -- 1243957
8) sometimes developers use special symbols in the name to structure the behavior of the method -- 975156
9) method names contains the name of a production method being called in the body; perform some stactic analysis on the method body -- 1137025
10) noun-verbs -- 221694
11) Failure of splitting (testInValidJDK) -- 18214
12) 829008 interesting example -- pack can be verb or noun depending on the context
13) good example of a bad rename -- 45881
14) good prepositional phrase example -- 1187161




Future research --
1) taggers should be intelligent to detect spelling mistakes in the terms making up the name before determining the term's part-of-speech tag --- 1058371
2) linguistic anti-patten smells based on grammar patterns
3) how to handle names that are prepend with specific 'keywords' e.g., IGNORE -- 602996 (preamble)



